Search for new phenomena in the WW to l nu l' nu' final state in pp collisions at sqrt(s) = 7 TeV with the ATLAS detector

This Letter reports a search for a heavy particle that decays to WW using events produced in pp collisions at sqrt(s) = 7 TeV. The data were recorded in 2011 by the ATLAS detector and correspond to an integrated luminosity of 4.7 fb-1. WW to l nu l' nu'(l, l' = e or mu) final states are considered and the distribution of the transverse mass of the WW candidates is found to be consistent with Standard Model expectations. Upper limits on the production cross section times branching ratio into W boson pairs are set for Randall-Sundrum and bulk Randall-Sundrum gravitons, which result in observed 95% CL lower limits on the masses of the two particles of 1.23 TeV and 0.84 TeV, respectively.

==> Makefile <==
LATEX    = latex
BIBTEX   = bibtex
DVIPS    = dvips

BASENAME = WWlvlv

default: testlatex

testlatex:
	latex  ${BASENAME}
	bibtex ${BASENAME}
	latex  ${BASENAME}
	latex  ${BASENAME}
#	latex  ${BASENAME}
	dvipdf -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}

testpdflatex:
	pdflatex  ${BASENAME}
	bibtex    ${BASENAME}
	pdflatex  ${BASENAME}
	pdflatex  ${BASENAME}
#	pdflatex  ${BASENAME}

#
# standard Latex targets
#

%.dvi:	%.tex 
	$(LATEX) $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

%.ps:	%.dvi
	$(DVIPS) $< -o $@

%.pdf:	%.tex
	$(PDFLATEX) $<

.PHONY: clean testpdflatex testlatex

clean:
	rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
	      *.inx *.dvi *.toc *.out *~ ~* spellTmp 


